Online Task Assignment with Controllable Processing Time

We study a new online assignment problem, called the Online Task Assignment with Controllable Processing Time. In a bipartite graph, a set of online vertices (tasks) should be assigned to a set of offline vertices (machines) under the known adversarial distribution (KAD) assumption. We are the first to study controllable processing time in this scenario: There are multiple processing levels for each task and higher level brings larger utility but also larger processing delay. A machine can reject an assignment at the cost of a rejection penalty, taken from a pre-determined rejection budget. Different processing levels cause different penalties. We propose the Online Machine and Level Assignment (OMLA) Algorithm to simultaneously assign an offline machine and a processing level to each online task. We prove that OMLA achieves $1/2$-competitive ratio if each machine has unlimited rejection budget and $\Delta/(3\Delta-1)$-competitive ratio if each machine has an initial rejection budget up to $\Delta$. Interestingly, the competitive ratios do not change under different settings on the controllable processing time and we can conclude that OMLA is "insensitive" to the controllable processing time.

==> [arXiv] OMLA (For Publish)/Sections/Analysis.tex <==
\section{Competitive Ratio Analysis}\label{sec:4}

 In this section, we analyze the competitive ratio of our online algorithm. The sketch of our analysis is shown in Figure \ref{fig:sketch}. We have already derived  Lemma~\ref{lm:1}, where we find an upper bound LP(\texttt{Off}) of the offline optimal value. Then we first introduce our reference system, which provides a lower bound of the original system (Lemma \ref{lm:22}). In this reference system, each task with $L$ levels are reconstructed as $L$ tasks with a single level. After Lemma \ref{lm:22}, we analyze the competitive ratio in two branches separately: \textcircled{1} each machine $u$ has an infinite initial rejection budget $\Delta_u=\infty$ (the unlimited rejection case); \textcircled{2} each machine $u$ has a finite rejection budget $\Delta_u<\infty$. For the unlimited rejection case, we first find a lower bound for the reference system (Lemma \ref{lm:3}). Then we construct the \textit{auxiliary inequality} for the unlimited rejection case (Lemma \ref{lm:4}) by Lemmas \ref{lm:1}--\ref{lm:3}. Then by Lemma \ref{lm:4}, we prove that OMLA is $1/2$-competitive for the unlimited rejection case (Theorem \ref{tr:1}). For the limited rejection case, we first find the \textit{performance induction inequality} of the reference system (Lemma \ref{lm:5}). With this inequality, we find a lower bound of the reference system (Lemma \ref{lm:6}). Then we construct the auxiliary inequality for the limited rejection case (Lemma \ref{lm:7}) by Lemmas \ref{lm:1}, \ref{lm:22}, and \ref{lm:6}. By Lemma \ref{lm:7}, we prove that OMLA is $\Delta/(3\Delta-1)$-competitive for the limited rejection case, where $\Delta=\max_{u\in U}\Delta_u$ (Theorem \ref{tr:2}).
 
 %, we analyze the competitive ratio in two branches separately: \textcircled{1} each machine $u$ has an infinite initial rejection budget (Lemmas \ref{lm:3}--\ref{lm:4} and Theorem \ref{tr:1}). \textcircled{2} each machine $u$ has a finite rejection budget. We first find a lower bound of the reference system (Lemmas \ref{lm:5}--\ref{lm:7} and Theorem \ref{tr:2}). 
 %A more detailed workflow of our analysis is shown in Appendix.


%Then we construct the \textit{auxiliary inequality} for the unlimited rejection case (Lemma \ref{lm:4}) by Lemmas \ref{lm:1}-\ref{lm:3}. Then by Lemma \ref{lm:4}, we prove that Algorithm \ref{alg:online} is $1/2$-competitive for the unlimited rejection case (Theorem \ref{tr:1}). For the limited rejection case, we first find the \textit{performance induction inequality} of the reference system (Lemma \ref{lm:5}). With Lemma \ref{lm:5}, we employee a similar approach to analyze the limited rejection case: lower bound of the reference system (Lemma \ref{lm:6} )and auxiliary inequality (Lemma \ref{lm:7}). By Lemma \ref{lm:7}, we prove that OMLA  is $\Delta/(3\Delta-1)$-competitive for the limited rejection case, where $\Delta=\max_{u\in U}\Delta_u$ (Theorem \ref{tr:2}).}


\begin{comment}


In this section, we analyze the competitive ratio of our online algorithm. The sketch of our analysis is shown in Figure \ref{fig:sketch}. We have already derived  Lemma~\ref{lm:1}, where we find an upper bound LP(\texttt{Off}) of the offline optimal value. 
%The analysis firstly follows Lemma 1, where we find an upper bound LP(\texttt{Off}) of the offline optimal value. 
After that, in this section, we first introduce our reference system, which provides a lower bound of the original system. In this reference system, each task with $L$ levels are reconstructed as $L$ tasks with a single level. Then the performance of the reference system is a lower bound of the original system (Lemma \ref{lm:2}). After Lemma \ref{lm:2}, we analyze the competitive ratio in two branches separately: 1) each machine $u$ has an infinite initial rejection budget $\Delta_u=\infty$ (the unlimited rejection case); 2) each machine $u$ has a finite rejection budget $\Delta_u<\infty$ (the limited rejection case). For the unlimited rejection case, we first find a lower bound of the reference system (Lemma \ref{lm:3}). Then we construct the \textit{auxiliary inequality} for the unlimited rejection case (Lemma \ref{lm:4}) by Lemmas \ref{lm:1}-\ref{lm:3}. Then by Lemma \ref{lm:4}, we prove that Algorithm \ref{alg:online} is $1/2$-competitive for the unlimited rejection case (Theorem \ref{tr:1}). For the limited rejection case, we first find the \textit{performance induction inequality} of the reference system (Lemma \ref{lm:5}). With this inequality, we find a lower bound of the reference system (Lemma \ref{lm:6}). Then we construct the auxiliary inequality for the limited rejection case (Lemma \ref{lm:7}) by Lemma \ref{lm:1}, Lemma \ref{lm:2} and Lemma \ref{lm:6}. By Lemma \ref{lm:7}, we prove that Algorithm \ref{alg:online} is $\Delta/(3\Delta-1)$-competitive for the limited rejection case, where $\Delta=\max_{u\in U}\Delta_u$ (Theorem \ref{tr:2}).

\begin{figure}{}
     \centering
         \includegraphics[width=0.45\textwidth]{sketch.png}
         
         \caption{Sketch of Analysis}
         \label{fig:sketch}
\end{figure}
\end{comment}
%Let us first introduce the reference system.

\begin{figure}[h!]{}
     \centering
         \includegraphics[width=0.95\textwidth]{sketch2.png}
         
         \caption{Sketch of Analysis.}
         \label{fig:sketch}
\end{figure}

\subsection{Reference System}\label{sec:4.1}

It is not straightforward to directly analyze the performance of the original system, so that we need to find an intermediate value to bound it. One key challenge of the original problem is introduced by different processing levels.  %this problem is rather a tripartite matching problem than a bipartite matching problem, where 
With controllable processing time, $L$ processing levels form one additional dimension. The reference system is to construct another bipartite matching system without this additional dimension, to provide a lower bound of the original tripartite matching system. We will also need to show: 1) the reference system is a valid system; and 2) the expected reward of this reference system is a valid lower bound for $R^{\Delta_u}_{u,1}$.

For each machine $u$, we construct a reference system for $u$ as follows. The reference system has a bipartite graph $G'_u=(U'_u,V'_u;E'_u,)$, where $U'_u$ contains only one machine $u$, $V'_u$ is a set of non-repeatable tasks. At each $t$, one of $L$ tasks may come, denoted by $v'_{u,l,t}$, with a probability $p'_{u,l,t}$. Each of $L\times T$ tasks in $V'_u$ is different from each other. $v'_{u,l,t}$ can only be processed with processing level $l$. Each $v'_{u,l,t}$ has an edge to $u$. If task $v'_{u,l,t}$ arrives at $t$ and $u$ is available, we must choose $u$ and we must decide whether to assign $u$ to $v'_{u,l,t}$. Suppose $u$'s remaining budget is $\delta$ at $t$. Similar to the baseline value and activation value (Section \ref{sec:3.4}), we define the reference baseline value (resp. the reference activation value) as $\Tilde{R}^\delta_{u,t}$ (resp., $\Tilde{Q}^\delta_{u,l,t}$). The calculation of reference baseline values and reference activation values is similar to that of baseline values and activation values,
and will be given shortly. We compare the reference activation value of $u$ at $t$ and the reference baseline value of $u$ at $t+1$. The higher one indicates our choice: If the former one is larger, we assign $u$ to $v'_{u,l,t}$; Otherwise, we discard $v'_{u,l,t}$. The probability that $u$ accepts this assignment is $q'_{u,l,t}$. The reward of processing $v'_{u,l,t}$ is $r'_{u,l,t}$. The processing time $d'_l$ is drawn from the known distribution $D_l$. The rejection penalty is $\theta_l$, same as in the original system. The initial budget of $u$ is $\Delta_u$, same as in the original system. We set the parameters $p'_{u,l,t}$, $q'_{u,l,t}$, and $r'_{u,l,t}$ in the reference system as follows:
The probability that $v'_{u,l,t}$ arrives at $t$: $p'_{u,l,t}=\sum_{e\in E_u}x^*_{e,l,t}$;
The probability that $u$ accepts the assignment of task $v'_{u,l,t}$: $q'_{u,l,t}=(\sum_{e\in E_u}q_ex^*_{e,l,t})/p'_{u,l,t}$ if $p'_{u,l,t}>0$; otherwise $q'_{u,l,t}=0$; The reward of processing $v'_{u,l,t}$ (with level $l$): $ r'_{u,l,t}=(\sum_{e\in E_u}q_er_{u,v,l}x^*_{e,l,t})/(p'_{u,l,t}q'_{u,l,t})$ if $p'_{u,l,t}q'_{u,l,t}>0$, otherwise $r'_{u,l,t}=0$.
The distribution of occupation time of processing level $l$ is $\text{Pr}\{d'_l=d\}=\text{Pr}\{d_l=d\}.$

With the above parameters, we can calculate $\Tilde{Q}^\delta_{u,l,t}$ and $\Tilde{R}^\delta_{u,t}$ by
\begin{align}
    \Tilde{R}_{u,t}^\delta=&\sum_{l\in\mathcal{L}}p'_{u,l,t}\max\{\Tilde{Q}^\delta_{u,l,t},\Tilde{R}^\delta_{u,t+1}\}
    +\Big(1-\sum_{l\in\mathcal{L}}p'_{u,l,t}\Big)\Tilde{R}^\delta_{u,t+1},\ \  (\delta>0,t\in[T])\label{eqn:18},\\
    \Tilde{Q}^\delta_{u,l,t}=&q'_{u,l,t}\Big(r'_{u,l,t}+\sum_{d'\in[T-t]}\text{Pr}\{d_l=d'\}\Tilde{R}^\delta_{u,t+d'}\Big)+(1-q'_{u,l,t})\Tilde{R}^{\delta-\theta_l}_{u,t+1},\ \ (\delta>0,t\in[T])\label{eqn:19}.
\end{align}
We set $\Tilde{R}_{u,t}^\delta=0$ and $\Tilde{Q}^\delta_{u,l,t}=0$ if $\delta\leq0$ or $t>T$. We note that we do not need to calculate the specific value of $\Tilde{Q}^\delta_{u,l,t}$ and $\Tilde{R}^\delta_{u,t}$ (no computational complexity is introduced). We only need the above values in the progress of the analysis. We note that the reference system for each $u$ is a valid system, because each $p'_{u,l,t}$ and $q'_{u,l,t}$ is a valid probability value. From (\ref{eqn:offst6}), we have $p'_{u,l,t}\leq1$ and $\sum_{l}p'_{u,l,t}\leq1$. From (\ref{eqn:offst1}), we have $q'_{u,l,t}\leq1$. Therefore, $p'_{u,l,t}$ and $q'_{u,l,t}$ are valid probability values and the reference system for each machine $u$ is a valid system.

In Lemma \ref{lm:22}, we show that for each $u$, $t$, and $\delta$, the performance of the reference system $\Tilde{R}_{u,t}^\delta$ is a lower bound of the performance of $u$ in the original system $R^\delta_{u,t}$.

\begin{lemma}
\label{lm:22}
(Reference System Bounds Original System)    $R_{u,t}^\delta\geq\Tilde{R}_{u,t}^\delta$, $\forall \delta$ and $t$.
\end{lemma}






By Lemma \ref{lm:22}, we can use the lower bound of $\Tilde{R}^\delta_{u,t}$ as a valid lower bound for $R^\delta_{u,t}$. With this reference system, we first analyze the competitive ratio when each machine has an infinite initial rejection budget, then analyze the competitive ratio when each machine has an initial rejection budget no more than $\Delta$, where $\Delta=\max_{u\in U} \Delta_u$. 


\begin{comment}

It is not straightforward to directly analyze the performance of the original system, so that we need to find an intermediate value to bound it. We notice that one key challenge of this problem is introduced by different processing levels. With controllable processing time, %this problem is rather a tripartite matching problem than a bipartite matching problem, where 
$L$ processing levels form one additional dimension. The motivation of the reference system is to construct another bipartite matching system without this additional dimension, to provide a lower bound of the original tripartite matching system. We will also need to show: 1) the reference system is a valid system; and 2) the expected reward of this reference system is a valid lower bound for $R^{\Delta_u}_{u,1}$. 

For each machine $u$, we construct a reference system for $u$ as follows. The reference system has a bipartite graph $G'_u=(U'_u,V'_u;E'_u,)$, where $U'_u$ contains only one machine $u$, $V'_u$ is a set of non-repeatable tasks. At each $t$, one of $L$ tasks may come, denoted by $v'_{u,l,t}$, with a probability $p'_{u,l,t}$. In total, we have $L\times T$ tasks in $V'_u$, and each of them is different from each other. For $v'_{u,l,t}$, it can only be processed with processing level $l$.
Each $v'_{u,l,t}$ has an edge to $u$. In other words, we have $V'_u=\{v'_{u,l,t}\ |\ l\in\mathcal{L},t\in[T]\}$ and $E'_u=\{(u,v')\ |\ v'\in V'_u\}$. If task $v'_{u,l,t}$ arrives at $t$ and $u$ is available, we must choose $u$ and we must decide whether to assign $u$ to $v'_{u,l,t}$. Suppose $u$'s remaining budget is $\delta$ at $t$. If $\delta\leq0$ or $u$ is occupied by a previous task, we  discard task $v'_{u,l,t}$. 
Similar to the baseline value and activation value (Section \ref{sec:3.4}), we define the reference baseline value of $u$ at $t$ as the expected sum reward of $u$ at and after $t$ before we know whether a task will arrive at $t$, which is denoted by $\Tilde{R}^\delta_{u,t}$. We define the reference activation value of $u$ at $t$ as the expected sum reward of $u$ at and after $t$ if $u$ is assigned to $v'_{u,l,t}$, which is denoted by $\Tilde{Q}^\delta_{u,l,t}$. 
The calculation of reference baseline values and reference activation values is similar to that of baseline values and activation values, and will be given shortly. We compare the reference baseline value of $u$ at $t+1$ and the reference activation value of $u$ at $t$, the higher one indicates our choice: If the former one is larger, we assign $u$ to $v'_{u,l,t}$; Otherwise, we discard $v'_{u,l,t}$.
%To decide whether to assign $u$ to $v'_{u,l,t}$, we compare two values: 1) the expected reward of $u$ if $u$ is assigned to $v'_{u,l,t}$ with level $l$, which is denoted by $\Tilde{Q}^\delta_{u,l,t}$; 2) the expected reward of $u$ if we do not make this assignment, which is equal to the expected reward of $u$ at time $t+1$, denoted by $\Tilde{R}^\delta_{u,t}$. The calculation of $\Tilde{Q}^\delta_{u,l,t}$ and $\Tilde{R}^\delta_{u,t}$ will be given later. If $\Tilde{Q}^\delta_{u,l,t}<\Tilde{R}^\delta_{u,t}$, we do not assign $v'_{u,l,t}$ to $u$ and discard $v'_{u,l,t}$. Otherwise, we assign $u$ to $v'_{u,l,t}$ with level $l$. 
With probability $q'_{u,l,t}$, $u$ accepts this assignment, immediately gets a reward $r'_{u,l,t}$, becomes occupied for a random period $d'_l$, and returns to the system at $t+d'_l$. $d'_l$ is drawn from the known distribution $D_l$. The initial budget of $u$ is the same as in the original system, which is $\Delta_u$. With probability $1-q'_{u,l,t}$, $u$ rejects that assignment, and takes a rejection penalty $\theta_l$ from its remaining budget $\delta$. We set the parameters $p'_{u,l,t}$, $q'_{u,l,t}$, $r'_{u,l,t}$ in the reference system as follows:
\\The probability that $v'_{u,l,t}$ arrives at $t$: 
    \begin{equation}
        p'_{u,l,t}=\sum_{e\in E_u}x^*_{e,l,t}
    \end{equation}
\\The probability that $u$ accepts the assignment of task $v'_{u,l,t}$: 
    \begin{equation}
        q'_{u,l,t}=\frac{\sum_{e\in E_u}q_ex^*_{e,l,t}}{p'_{u,l,t}}
    \end{equation}
    if $p'_{u,l,t}>0$, otherwise $q'_{u,l,t}=0$\\
\\The reward of processing $v'_{u,l,t}$ (with level $l$): 
    \begin{equation}
        r'_{u,l,t}=\frac{\sum_{e\in E_u}q_er_{u,v,l}x^*_{e,l,t}}{p'_{u,l,t}q'_{u,l,t}}
    \end{equation}
    if $p'_{u,l,t}q'_{u,l,t}>0$, otherwise $r'_{u,l,t}=0$;\\
\\The distribution of occupation time of processing level $l$: 
    \begin{equation}
        \text{Pr}\{d'_l=d\}=\text{Pr}\{d_l=d\}.
    \end{equation}

   \begin{itemize}
    \item The probability that $v'_{u,l,t}$ arrives at $t$: 
    \begin{equation}
        p'_{u,l,t}=\sum_{e\in E_u}x^*_{e,l,t}
    \end{equation}
    \item The probability that $u$ accepts the assignment of task $v'_{u,l,t}$: 
    \begin{equation}
        q'_{u,l,t}=\frac{\sum_{e\in E_u}q_ex^*_{e,l,t}}{p'_{u,l,t}}
    \end{equation}
    if $p'_{u,l,t}>0$, otherwise $q'_{u,l,t}=0$
    \item The reward of processing $v'_{u,l,t}$ (with level $l$): 
    \begin{equation}
        r'_{u,l,t}=\frac{\sum_{e\in E_u}q_er_{u,v,l}x^*_{e,l,t}}{p'_{u,l,t}q'_{u,l,t}}
    \end{equation}
    if $p'_{u,l,t}q'_{u,l,t}>0$, otherwise $r'_{u,l,t}=0$;\\
    \item The distribution of occupation time of processing level $l$: 
    \begin{equation}
        \text{Pr}\{d'_l=d\}=\text{Pr}\{d_l=d\}.
    \end{equation}
\end{itemize} 

With the above parameters, we can calculate $\Tilde{Q}^\delta_{u,l,t}$ and $\Tilde{R}^\delta_{u,t}$ by
\begin{align}
    \Tilde{R}_{u,t}^\delta=&\sum_{l\in\mathcal{L}}p'_{u,l,t}\max\{\Tilde{Q}^\delta_{u,l,t},\Tilde{R}^\delta_{u,t+1}\}\nonumber\\
    &+\Big(1-\sum_{l\in\mathcal{L}}p'_{u,l,t}\Big)\Tilde{R}^\delta_{u,t+1},\ \  (\delta>0,t\in[T])\label{eqn:18},
\end{align}
and
\begin{align}
    \Tilde{Q}^\delta_{u,l,t}=&q'_{u,l,t}\Big(r'_{u,l,t}+\sum_{d'\in[T-t]}\text{Pr}\{d_l=d'\}\Tilde{R}^\delta_{u,t+d'}\Big)\nonumber\\&+(1-q'_{u,l,t})\Tilde{R}^{\delta-\theta_l}_{u,t+1},\ \ (\delta>0,t\in[T])\label{eqn:19}.
\end{align}
Similarly, we set $\Tilde{R}_{u,t}^\delta=0$ and $\Tilde{Q}^\delta_{u,l,t}=0$ if $\delta\leq0$ or $t>T$. We note that we do not need to calculate the specific value of $\Tilde{Q}^\delta_{u,l,t}$ and $\Tilde{R}^\delta_{u,t}$ (no computational complexity is introduced). We only need the above values in the progress of the analysis.

We note that the reference system for each $u$ is a valid system, because each $p'_{u,l,t}$ and $q'_{u,l,t}$ is a valid probability value. From (\ref{eqn:offst6}), we have $p'_{u,l,t}\leq1$ and $\sum_{l}p'_{u,l,t}\leq1$. From (\ref{eqn:offst1}), we have $q'_{u,l,t}\leq1$. Therefore, $p'_{u,l,t}$ and $q'_{u,l,t}$ are valid probability values. The reference system for each machine $u$ is a valid system.

In Lemma \ref{lm:2}, we show that for each $u$, $t$ and $\delta$, the performance of the reference system $\Tilde{R}_{u,t}^\delta$ is a lower bound of the performance of $u$ in the original system $R^\delta_{u,t}$.

\begin{lemma}
\label{lm:2}
(Reference System Bounds Original System)    $R_{u,t}^\delta\geq\Tilde{R}_{u,t}^\delta$, $\forall \delta$ and $t$
\end{lemma}





By Lemma \ref{lm:2}, we can use the lower bound of $\Tilde{R}^\delta_{u,1}$ as a valid lower bound for $R^\delta_{u,t}$. With this reference system, we first analyze the competitive ratio when each machine has an infinite initial rejection budget, then analyze the competitive ratio when each machine has an initial rejection budget no more than $\Delta$, where $\Delta=\max_{u\in U} \Delta_u$. 

\end{comment}

\subsection{Unlimited Rejection Case}\label{sec:4.2}

In this section, we analyze the competitive ratio for the unlimited rejection case. In the unlimited rejection case, each $u$ has an infinite initial rejection budget $\Delta_u=\infty$. One straightforward way is to let $\Delta_u$ to be sufficiently large when we run Algorithms \ref{alg:online} and \ref{alg:QR}. A more efficient way is to replace $R_{u,t}^{\delta}$, $Q_{e,l,t}^\delta$, $\Tilde{R}_{u,t}^\delta$, and $\Tilde{Q}_{u,l,t}^\delta$ ($\forall \delta$) by  $R_{u,t}$, $Q_{e,l,t}$, $\Tilde{R}_{u,t}$, and $\Tilde{Q}_{u,l,t}$ respectively as they are indifferent under different $\delta$. The slightly modified Algorithms \ref{alg:online} and \ref{alg:QR} are shown in the Appendix. 

%We denote $\Tilde{R}_{u,t}=\Tilde{R}^\infty_{u,t}$ and $\Tilde{Q}_{u,l,t}=\Tilde{Q}^\infty_{u,l,t}$. 


%{One straightforward is to let $\Delta_u$ to be sufficiently large when we run Algorithms X and x. A more efficient way is to we can also remove the superscript in Algorithm $R_{u,t}=R^\infty_{u,t}$ 


% \color{blue} Similarly, we can denote $R_{u,t}=R^\infty_{u,t}$ and $Q_{u,l,t}=Q^\infty_{u,l,t}$, so that we do not need to memory the remaining budget of $u$ in Algorithm \ref{alg:online}, or the dimension of $\delta$ for Q-value and R-value in Algorithm \ref{alg:online} and Algorithm \ref{alg:QR}} 

The main result of this section is that Algorithm \ref{alg:online} is $1/2$-competitive for the unlimited rejection case (Theorem \ref{tr:1}). To get this result, we first get a lower bound of the performance of the reference system (Lemma \ref{lm:3}), then construct an auxiliary inequality (Lemma \ref{lm:4}) to show that a lower bound of the competitive ratio can be obtained by the ratio between the lower bound of $\sum_{u}\Tilde{R}_{u,1}$ and the offline optimal value LP(\texttt{Off}). Finally, by Lemma \ref{lm:4}, we get the result in Theorem \ref{tr:1}.

We first show that we have a lower bound for $\Tilde{R}_{u,1}$ in Lemma \ref{lm:3}.  $\Tilde{R}_{u,1}$ is $u$'s expected sum reward at and after $t=1$ (overall expected sum reward of $u$) in the reference system.

\begin{lemma}
\label{lm:3} (Reference System Lower Bound)
    For each $u$, we have 
    \begin{equation}
        \Tilde{R}_{u,1}\geq\frac{1}{2}\sum_{t\in[T]}\sum_{l\in\mathcal{L}}\sum_{e\in E_u}q_er_{u,v,l}x^*_{e,l,t}\label{eq4:16}.
    \end{equation}
\end{lemma}


To prove Lemma \ref{lm:3}, the key step is to establish a dual LP to derive the bound.  We also utilize the property that ``the sum of maximum is no less than the maximum of sum''. Next, we show the auxiliary inequality for the unlimited case by Lemmas \ref{lm:1}--\ref{lm:3}.
\begin{lemma}
\label{lm:4} (Auxiliary  Inequality)
    For the original system, in the unlimited rejection case, we have
    \begin{align}
        \frac{\mathbb{E}_{I\sim\mathcal{I}}[\text{ALG}(I)]}{\mathbb{E}_{I\sim\mathcal{I}}[\text{OPT}(I)]}\geq\frac{\frac{1}{2}\displaystyle{\sum_{u\in U}\sum_{t\in[T]}\sum_{l\in\mathcal{L}}\sum_{e\in E_u}}q_er_{u,v,l}x^*_{e,l,t}}{\text{LP}(\texttt{Off})}.
    \end{align}
\end{lemma}


 Then we introduce Theorem \ref{tr:1}. We prove that Algorithm \ref{alg:online} is $1/2$-competitive for the unlimited rejection case.

\begin{theorem}
\label{tr:1}(Competitive Ratio of Unlimited Rejection)
    OMLA is $1/2$-competitive for the problem with unlimited rejection budget.
\end{theorem}

\subsection{Limited Rejection Case}\label{sec:4.3}

In this section, we analyze the competitive ratio for the limited rejection case. Each $u$ has a finite initial rejection budget $\Delta_u<\infty$. The main result of this subsection is that Algorithm \ref{alg:online} is $\Delta/(3\Delta-1)$-competitive for the limited rejection case, where $\Delta=\max_{u\in U}\Delta_u$ (Theorem \ref{tr:2}). To get this result, we first present performance induction inequality (Lemma \ref{lm:5}), which is used to get a lower bound of the performance of the reference system (Lemma \ref{lm:6}). Then we construct an auxiliary  inequality (Lemma \ref{lm:7}) to show that a lower bound of the competitive ratio can be obtained by the ratio between the lower bound of $\sum_u\Tilde{R}_{u,1}^{\Delta_u}$ and the offline optimal value LP(\texttt{Off}). Finally, by Lemma \ref{lm:7}, we conclude the result in Theorem \ref{tr:2}.

We first show an inequality on $\Tilde{R}_{u,t}^{\delta-\theta_l}$ and $\Tilde{R}_{u,t}^\delta$, which is used to get a lower bound of the performance of the reference system. Please note that this inequality is new for the limited rejection as we need to consider the remaining budget $\delta$ now.

\begin{lemma} \label{lm:5}(Performance Induction Inequality)
    For all $\delta$, $t$ and $l$, we have
    \begin{equation}
        \Tilde{R}_{u,t}^{\delta-\theta_l}\geq\frac{\delta-\theta_l}{\delta}\Tilde{R}_{u,t}^\delta.\label{eq3:42}
    \end{equation}
\end{lemma}


Then we show that we have a lower bound for $\Tilde{R}_{u,1}^{\Delta_u}$.
\begin{lemma} \label{lm:6}(Reference System Lower Bound)
    For each $u$, we have
    \begin{equation}
        \Tilde{R}_{u,1}^{\Delta_u}\geq\frac{\Delta_u}{3\Delta_u-1}\sum_{t\in[T]}\sum_{l\in\mathcal{L}}\sum_{e\in E_u}q_er_{u,v,l}x^*_{e,l,t}.
    \end{equation}\label{eq4:19}
\end{lemma}


 The key step is to establish a dual LP to derive the bound. By Lemma \ref{lm:6}, we can eliminate the influence of different rejection penalty values (non-homogeneous $\theta_l$) of different levels from (\ref{eq4:19}). %To achieve this, we utilize the inequality in (\ref{eqn:offst2}) in the analysis. %Recall that in (\ref{eqn:offst2}), we use the initial budget to restrict the machines' rejection, but allow each machine to slightly overdraw its budget a little (a machine may reject an assignment with a rejection penalty higher that its remaining budget). 
In the proof, it is sufficient to derive a bound utilizing the dual LP, and the dual LP can eliminate the impact of non-homogeneous $\theta_l$ in (\ref{eqn:offst2}). %Compared to the design where machines are not allowed to overdraw its budget, this design is able to handle non-homogeneous $\theta_l$.% has two advantages: 1) First, it makes LP(\texttt{Off}) closer to the offline optimal value; 2) Second, it allows our online algorithm to have a higher performance.  

Next, we show the auxiliary inequality for the limited rejection case by Lemmas \ref{lm:1}, \ref{lm:22}, and \ref{lm:6}. 

\begin{lemma} \label{lm:7} (Auxiliary  Inequality)
    For the original system, under the limited rejection case, we have
    \begin{equation}
        \frac{\mathbb{E}_{I\sim\mathcal{I}}[\text{ALG}(I)]}{\mathbb{E}_{I\sim\mathcal{I}}[\text{OPT}(I)]}\geq\frac{\displaystyle{\sum_{u\in U}\frac{\Delta_u}{3\Delta_u-1}\sum_{t\in[T]}\sum_{l\in\mathcal{L}}\sum_{e\in E_u}}q_er_{u,v,l}x^*_{e,l,t}}{\text{LP}(\texttt{Off})}.
    \end{equation}
\end{lemma}

Then we introduce Theorem \ref{tr:2}. We prove that OMLA is $\Delta/(3\Delta-1)$-competitive for the limited rejection case, where $\Delta=\max_{u\in U}\Delta_u$.
\begin{theorem}
\label{tr:2}
    OMLA is a $\Delta/(3\Delta-1)$-competitive algorithm for the limited rejection case, where $\Delta=\max_{u\in U}\Delta_u$.
\end{theorem}


\begin{comment}

\begin{figure*}
\subfigure{\includegraphics[width=0.24\textwidth]{figures/fig1_0116.jpg}}
         \label{fig:1a}
\hspace{0.01\textwidth}
\subfigure{\includegraphics[width=0.24\textwidth]{figures/fig1_0116.jpg}}
\caption{Online Performance / LP(\texttt{Off}) of different $L$ and $\Delta$.}
        \label{fig:2}

\end{figure*}

\end{comment}

\begin{comment}

\begin{figure*}[t]
     \centering
     \begin{subfigure}{0.24\columnwidth}
         
         \includegraphics[width=\linewidth]{figures/fig1_0116.jpg}
         
         \caption{Online / LP(\texttt{Off}), $L$=6}
         \label{fig:1a}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         
         \includegraphics[width=\textwidth]{figures/fig2_0116.jpg}
         \caption{Online / LP(\texttt{Off}), $L$=12}
         \label{fig:1b}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         
         \includegraphics[width=\textwidth]{figures/fig3_0116.jpg}
         \caption{Online / LP(\texttt{Off}), $\Delta$=20}
         \label{fig:1c}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         
         \includegraphics[width=\textwidth]{figures/fig4_0116.jpg}
         \caption{Online / LP(\texttt{Off}), $\Delta$=$\infty$}
         \label{fig:1d}
     \end{subfigure}
        \caption{Figure 2: Online Performance / LP(\texttt{Off}) of different $L$ and $\Delta$.}
        \label{fig:2}
\end{figure*}

\begin{figure*}[t]
     \centering
     \begin{subfigure}{0.24\textwidth}
         
         \includegraphics[width=\textwidth]{figures/fig5_4_0116.jpg}
         
         \caption{Online / LP(\texttt{Off}), $L$=6}
         \label{fig:2a}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         
         \includegraphics[width=\textwidth]{figures/fig6_1_0116.jpg}
         \caption{Online / LP(\texttt{Off}), $L$=12}
         \label{fig:2b}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         
         \includegraphics[width=\textwidth]{figures/fig7_4_0116.jpg}
         \caption{Online / LP(\texttt{Off}), $\Delta$=20}
         \label{fig:2c}
     \end{subfigure}
     \begin{subfigure}{0.24\textwidth}
         
         \includegraphics[width=\textwidth]{figures/fig8_1_0116.jpg}
         \caption{Online / LP(\texttt{Off}), $\Delta$=$\infty$}
         \label{fig:2d}
     \end{subfigure}
        \caption{Figure 3: Online Performance / LP(\texttt{Off}) of different benchmarks with different $L$ and $\Delta$.}
        \label{fig:3}
\end{figure*}
\end{comment}


==> [arXiv] OMLA (For Publish)/Sections/Conclusion.tex <==
\section{Conclusion}\label{sec:6}

In this paper, we investigate the online bipartite matching problem with controllable processing time, motivated by real-world scenarios. We design OMLA, an online algorithm to simultaneously assign an offline machine and a processing level to each online task. We prove that OMLA achieves $1/2$-competitive ratio if each machine has unlimited rejection budget and $\Delta/(3\Delta-1)$-competitive ratio if each machine has an initial budget up to $\Delta$. Furthermore, we conduct experiments on synthetic data sets, where the results demonstrate that OMLA outperforms benchmarks under a variety of environments.

==> [arXiv] OMLA (For Publish)/Sections/Evaluation.tex <==
\section{Evaluation}\label{sec:5}


%\begin{figure}[t]
%    \centering
%    \subfigure[$L$=12]{\label{fig:2b}
%        \includegraphics[width=0.35\linewidth]{figure0119/fig6_0119.jpg}
%    }\hspace{-5.5mm}
%    \subfigure[$\Delta$=20]{\label{fig:2c}
%        \includegraphics[width=0.35\linewidth]{figure0119/fig7_2_0119.jpg}
%    }\hspace{-5.5mm}
%    \subfigure[$\Delta$=$\infty$]{\label{fig:2d}
%        \includegraphics[width=0.35\linewidth]{figure0119/fig8_0119.jpg}
%    }\hspace{-5.5mm}
%    \caption{Online Reward / LP(\texttt{Off}) of different benchmarks with different $L$ and $\Delta$.}
%    \label{fig:3}
%\end{figure}



%In this section, we present the evaluation of OMLA. We first introduce our benchmarks and synthetic data set. Then we present our simulation and real-world experiment.

\subsection{Benchmarks}\label{sec:5.1}

In this section, we evaluate OMLA against five benchmarks: 1) Random (R): the system randomly chooses a machine-level pair when an online task arrives. If the chosen machine is available, we assign this machine-level pair. Otherwise, we discard the task. 2) Utility Greedy (UG): when task $v$ arrives, the system ranks all the machine-level pairs by $r_{u,v,l}$ and chooses the highest one available. 3) Efficiency Greedy (EG): with the expectation $\mathbb{E}[d_l]$ of the occupation time of processing level $l$ calculated in advance, when task $v$ arrives, the system ranks all the machine-level pair by $r_{u,v,l}/\mathbb{E}[d_l]$ and chooses the highest one available. 4) Utility Greedy + (UG+): when a task $v$ arrives, we choose a machine $u$ by \cite{RN51}, then choose the level $l$ with the highest $r_{u,v,l}$. 5) Efficiency Greedy + (EG+): when a task $v$ arrives, we choose a machine $u$ by \cite{RN51}, then choose the level $l$ with the highest $r_{u,v,l}/\mathbb{E}[d_l]$. Please note that that \cite{RN51} did not consider processing level. We use the approach in \cite{RN51} to choose machine and then use greedy method to choose level in UG+ and EG+. 

\subsection{Synthetic Dataset}\label{sec:5.2}

We generate the synthetic data set in the experiment. (The approach was also adopted in \cite{RN51}.)  We set $|U|=10$, $|V|=25$, and $T=100$. For each $u$ and $v$, an edge $(u,v)$ exists in $E$ with probability $0.1$. For each $e\in E$, we set $q_e\sim U(0.5,1)$ and $r_{u,v,l}\sim U(a\cdot l^{0.2},a\cdot l^{0.4})$, where $a\sim U(0.5,1)$. For each $l\in\mathcal{L}$ we set the distribution $D_l$ as a binomial distribution $B(T,l^{1.2}/20)$. For settings (a), (b) in Figure 2 and (a) (b) in Figure 3, $\Delta_u$ is drawn uniformly from $[\Delta]$. We set the rejection penalty for level $l$ as $\theta_l=l+2$.

\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{figure0119/fig2_0119.jpg}
    \subcaption{$L$=12}
    \label{fig:1b}
    \end{minipage}
    \hspace{-5.5mm}
    \begin{minipage}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{figure0119/fig3_0119.jpg}
    \subcaption{$\Delta$=20}
    \label{fig:1c}
    \end{minipage}
    \hspace{-5.5mm}
    \begin{minipage}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{figure0119/fig4_0119.jpg}
    \subcaption{$\Delta$=$\infty$}
    \label{fig:1d}
    \end{minipage}
    
    \caption{Online Reward / LP(\texttt{Off}) of different $L$ and $\Delta$.}
    \label{fig:2}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{figure0119/fig6_0119.jpg}
    \subcaption{$L$=12}
    \label{fig:2b}
    \end{minipage}
    \hspace{-5.5mm}
    \begin{minipage}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{figure0119/fig7_2_0119.jpg}
    \subcaption{$\Delta$=20}
    \label{fig:2c}
    \end{minipage}
    \hspace{-5.5mm}
    \begin{minipage}[b]{0.33\linewidth}
    \includegraphics[width=\linewidth]{figure0119/fig8_0119.jpg}
    \subcaption{$\Delta$=$\infty$}
    \label{fig:2d}
    \end{minipage}
    
    \caption{Online Reward / LP(\texttt{Off}) of different benchmarks with different $L$ and $\Delta$.}
    \label{fig:3}
\end{figure}

\subsection{Verification of the Competitive ratio}\label{sec:5.3}

In Figure \ref{fig:2}, we investigate the ratio between the online performance of OMLA and LP(\texttt{Off}). We randomly generate a set of $\{p_{v,t}\}$, $E$ and $\{q_e\}$ for each sub-figure. For each pair of $\Delta$ and $L$, we generate a set of $\{\Delta_u\}$ and $\{r_{u,v,l}\}$, then we run $50$ rounds of experiment. In each round of experiment, we randomly generate $50$ task sequences from $\{p_{v,t}\}$, and calculate the ratio between the averaged total reward of OMLA and LP(\texttt{Off}). The orange bars in Figure \ref{fig:2} represent the competitive ratio of OMLA for each pair of $\Delta$ and $L$. The red dots in Figure \ref{fig:2} show the ratio between the averaged online total reward and LP(\texttt{Off}). Figure \ref{fig:2} shows that the ratio between the averaged performance of OMLA is indeed higher than the theoretical lower bound of the competitive ratio. The results in Figure \ref{fig:2} verifies our conclusion on the competitive ratios.

\subsection{Comparison of OMLA and Benchmarks}\label{sec:5.4}

In Figure \ref{fig:3}, we compare the performance of OMLA with benchmarks. We randomly generate a set of $\{p_{v,t}\}$, $E$ and $\{q_e\}$ for each sub-figure. For each pair of $\Delta$ and $L$, we generate a set of $\{\Delta_u\}$ and $\{r_{u,v,l}\}$. Then for each algorithm, we randomly generate $250$ task sequences from $\{p_{v,t}\}$, and calculate the ratio between the averaged total reward with LP(\texttt{Off}). OMLA outperforms all of the benchmarks with each pair of $\Delta$ and $L$. In Figures \ref{fig:2c} and \ref{fig:2d}, the performance of OMLA is slightly higher than the performance of UG+ and EG+ when the number of processing level is 2, but the performance gain becomes larger when there there are more processing levels. This demonstrates that OMLA is more advantageous for more processing levels as it is designed for joint assignment of machine and level. The results demonstrate that OMLA has the best performance with controllable processing time. OMLA provides both theoretical performance guarantees (competitive ratio) and the best average performance on the synthetic dataset.

==> [arXiv] OMLA (For Publish)/Sections/Introduction.tex <==
\section{Introduction}\label{sec:1}
In this paper, we study an online task assignment problem with controllable processing time. In this problem, we have a set of online vertices (tasks) and a set of offline vertices (machines). Online tasks arrive sequentially and each can be processed by a machine, but each task can only be processed by a subset of machines~\cite{RN49,RN51}. 
We focus on the controllable processing time: Each task has multiple levels of processing time~\cite{RN81,RN68}. If a task is processed with a higher level, it obtains a higher reward, but needs to wait for a longer time. %Each machine can only process one task at one time, and can only take another after the previous one is finished.
Each machine can only process one task at one time, and can only take another after the previous one is finished.
The machines do not always accept task assignment, and they lose an amount of rejection budget every time they reject. The higher processing level of the rejected assignment is, the larger amount of the budget is taken. When a machine runs out of its rejection budget, it will be removed from the system immediately and permanently. In this paper, we consider the online tasks arriving under \textit{known adversarial distributions} (KAD)~\cite{RN49,RN61}. The arrival probability of each task  at each time is known ahead. The goal is to maximise the expected reward %for known task sequences (offline setting) and 
without the knowledge of future task arrivals (online setting). 

Although a number of works have studied the online assignment problem, this paper is the first to consider controllable processing time. This is motivated by real-world scenarios in various fields, such as:
%This is motivated by a wide range of real-world scenarios, and there are several examples in different areas as follows. 

%In recent years, with the increasing variety of customer demands, controllable processing level has emerged among different fields. Traditionally, if several customer order a same service from a same vendor, they will get the service of a similar quality with a similar cost. However, not all customers expects a homogeneous quality of service or wants to bear a same cost, so a better strategy for the vendor is to provide a premium (resp., essential) version of the service for a higher (resp., lower) cost. This more flexible solution is what CSL is. Generally speaking, CSL becomes popular because it has the potential to better satisfy the customers with various demands of a single service.

%In this paper, we focus on the CSL emerged in the well-known bipartite matching problem. In the bipartite matching problem, there are two groups of entities, one presenting the demand side and another is the supply side. Traditionally, once an entity from the demand side expresses interests, we need to find an entity from the supply side to satisfied it, but with a fixed service level. With CSL, we can further choose to provide a better service for a higher satisfaction, or a more basic one to finish sooner. We can find this new service model in a wide range of real-world scenarios, and some examples are given as follows.

\textbf{1. Task offloading in edge computing}~\cite{RN63}. With the help of edge computing, end user devices can offload computing intensive tasks to edge computers, especially the ones processing machine learning (ML) models. Each user (task) has only a set of edge computers (machines)  near them, so the tasks from this user can only be processed by these computers. When we assign an edge computer to a task, we can further control the processing time by implementing different ML models. A better processing quality requires a model with longer processing time, but a lightweight  model (e.g., a pruned and sparsified model) finishes sooner, with lower accuracy. %The goal of edge computer assignment is to maximize users' total satisfaction. 

\textbf{2. Ride-sharing with tolls}~\cite{RN62}. Ride-sharing system assigns passenger requests (tasks) to available drivers (machines). Each request has an origin and can only be processed by drivers near this area. For each ride, we can choose to go through toll roads (high cost) for a shorter processing time, or to avoid toll for less cost. %To goal is to maximize the total net profit.

\textbf{3. Translation service}~\cite{RN85}. Customers place orders (tasks) to the language service agencies (machines), and the agency can provide different degrees of service (e.g., one-off translation, translation and proofreading, etc.). Each translation request has a target language and can only be processed by translators with a certification of this language. The agency can choose to assign more time for a translation task, resulting in a higher processing quality; but the agency can also assign a shorter processing time to a task, so that more customer requests can be processed.
%If the agency assigns a longer processing time to a translation task, the translation comes with a better quality; but the agency can also assign a shorter processing time to a task, so that more customer requests can be processed. %The goal of this  translation assignment problem is to balance between the number of processed requests and the translation quality, so that a maximized total utility can be achieved.

%Motivated by practical applications, we consider the online assignment problem with controllable processing times in this paper. Similar to the traditional online assignment problem, we have a finite time horizon and a bipartite graph. In this bipartite graph, one group of nodes represents available machines and another group represents online tasks. An online task may come at each moment, and we assign it to a machine with a processing level to gain a reward. Every time a machine is assigned, it can either reject the assignment with a fixed probability and remove a penalty from its budget, or accept it and becomes unavailable for a random period. In this paper, we consider both offline and online settings.  In the offline setting, we assume that the full arrival sequence of tasks is known ahead and we maximise the expected reward over all possible task sequences. In the online settings, with only the knowledge of the probability of each task arriving at each time, we design an algorithm to assign the arriving task to a machine with a processing time. 

In many situations, because the arrival of tasks can only be known when they arrive, online algorithms are required. We are motivated to design such an online algorithm that can maximize the worst ratio against the offline optimal performance (competitive ratio). In short, the online assignment problem studied in this paper has the following features:\\
\textbf{A. Known adversarial distribution (KAD):} the probability of the arrival of each task at each time is known in advance.\\
\textbf{B. Reusable machines:} the machine returns to the system after completing a task; the processing delay is drawn from known distributions.\\
\textbf{C. Controllable processing time:} each task can be processed with different levels; a higher processing level generates a higher reward but the expected delay is also higher.\\
\textbf{D. Budgeted machine rejections:} when a machine is assigned, it can reject the assignment with a penalty; rejecting a higher processing level task will cause higher penalty. 
When the budget runs out, the machine is permanently removed from the system.

The main contribution of this paper is designing an Online Machine and Level Assignment (OMLA) Algorithm for the above problem, especially with multiple processing levels. We  prove that our algorithm achieves a $1/2$-competitive ratio when every machine has an infinite rejection budget, and a $\Delta/(3\Delta-1)$-competitive ratio when each machine has a finite rejection budget, where $\Delta$ is the largest budget of machines at the beginning. The conclusion shows that regardless of the limited rejection budgets, the competitive ratio does not depend on the  processing levels, indicating that OMLA is insensitive to controllable processing time.

Controllable processing time makes the problem studied in the paper more realistic but also introduces substantially more challenges to the online algorithm design and competitive analysis. Controllable processing time expands the searching space. Since each processing level causes different rewards, delays, and rejection budgets. The algorithm should balance these dimensions as a result of coupled objective and constraints. To tackle this challenge, in our online algorithm design, we first use the joint probabilities of choosing a machine and  a level as decision variables to formulate an offline linear programming (LP). The optimal solution to the LP is then leveraged to calculate the activation value and the baseline value for each machine and level. These two values will determine our decision on the machine and level when we make decisions online. To bound the competitive ratio, we introduce a reference system where each task with $L$ levels are reconstructed as $L$ tasks with a single level. Then the performance of the reference system is employed as an intermediate value to bound the competitive ratio. Mathematical derivations demonstrate that multiple processing levels do not worsen the competitive ratio because the reference system uniformly bounds different processing levels, and thus the competitive ratio is insensitive to the controllable processing time.




% What's worse, with the increase of the number of possible processing levels, this selection base becomes even larger, which suggests a higher difficulty to properly assign a task and, consequently, a worse competitive ratio. However, even with controllable processing levels, we prove that our online algorithm achieves a same competitive ratio as good as a previous work({\color{red} aaai}),  which does not consider controllable processing levels. 


%We make several innovative design to eliminate the impact brought by controllable processing levels. First, to achieve the offline optimal value, we design constraint (\ref{eqn:offst2}) in the linear programming \texttt{Off}. This constraint brings different rejection penalty of different processing levels in to the system, but when we treat the "permanent occupation" as introducing the highest penalty to the machine, we can make the upper bound of the offline optimal value lower (closer to the offline optimal value). This design takes effects in the proof of lemma 5. Another design is in the reference system. Different from the original system, we only allow each task in the reference system to be processed with one processing level. With this design, we reserve the different processing levels in the system, but reduce the impact of it. This reduced impact is further eliminated when we construct inequalities, as in (\ref{eq2:21}) and in (\ref{eq2:31}).

%Before the design of an online algorithm, we need to construct an offline linear program, which aligns with the problem constraints and gives an upper bound of the offline expected reward. This is similar to the online assignment problem in {\color{red}(aaai)}, where each time at most one unit of budget will be taken for rejection. However, our problem setting allows different amount of penalty at different time, which requires a new constraint to avoid any negative remaining budget.

%In the online algorithm, we need to choose a machine $u$ with a processing level $l$. This is, actually, a tripartite matching problem. However, a tripartite matching algorithm is far more complex to design and analyze than a bipartite matching problem. We observed that, from the offline solution $x^*_{e,l,t}$ we can construct the probability that machine $u$ is assigned when $v$ arrives. Then by a conditional probability, we can further generate the joint probability that machine $u$ is assigned with processing level $l$ when $v$ arrives. This solution successfully avoid a complex tripartite algorithm but still provide a proper probability to choose the machine-level pair $(u,l)$.

%The most challenging part is how to construct a modified system. This modified system serves two main purposes: First, it is simplified system compared to the original one, which make it possible to do mathematical analysis; Second, it inherits the parameter of the original system in its own, which is utilised when giving the competitive ratio. The first purpose requires the deletion of some system feature of the original one, while the second requires to keep the parameters of those deleted features remained in reserved ones. The challenge comes right from this contradiction. We tried different solutions but only one works properly. In our modified system, there are still multiple possible tasks to come at each time. However, for each task we only allow one possible processing level. With this design, we greatly reduce the selection space upon the arrival of each task, but reserve a summation among the $L$ processing levels in the expected reward. One of the plausible but inferior solution we have tried is that, in the modified system, we allow only one possible task to come at each time but with $L$ possible processing levels, which would finally lead to a $1/(2L)$-competitive ratio even for the unlimited rejection cases.

%The rest of this paper is organised as follows: Section 2 gives a formal definition of the problem setting, constructs a linear programming \texttt{Off} to get a upper bound of the offline optimal value, and proposes our online algorithm. Section 3 analyzes the competitive ratio of our online algorithm. Subsection 3.1 explains how do we construct a reference system, why it is feasible and why it provides a lower bound for the original system. Subsection 3.2 analyzes the competitive ratio in unlimited rejection cases. Subsection 3.3 analyzes the competitive ratio in limited rejection cases.


==> [arXiv] OMLA (For Publish)/Sections/Model.tex <==
\section{Model}\label{sec:3}

We present a formal description of our problem in this section.  We have a bipartite graph $G=(U,V;E)$, where $U$ is the set of machines and $V$ is the set of repeatable tasks.\footnote{Please note that  $v\in V$ is actually indicating a type of tasks, which  arrive repeatably at different time. For presentation convenience and following the convention, $v$ is also called ``a task'' throughout this paper.} $E$ is the set of edges indicating if a task $v\in V$ can be processed by a machine $u\in U$. For each task, we have $L$ processing levels $\mathcal{L}=\{1,...,L\}$, indicating the $L$ quality levels. If task $v$ is processed by machine $u$ ($(u,v)\in E$) with processing level $l$, it will generate a reward of $r_{u,v,l}$. Without loss of generality (WLOG), we have $ r_{u,v,l}<r_{u,v,l'}$ when $l<l'$ (larger processing level gives larger reward). The system runs on a finite time horizon $T\in \mathbb{N}^+$. Each processing level $l\in\mathcal{L}$ causes a random processing delay $d_l$, which presents the occupation time to process a task with level $l$. In other words, if a machine  starts to process a task with level $l$, it becomes unavailable to any other tasks until time $t+d_l$. $d_l$ is drawn from a known distribution $D_l$. We have $\mathbb{E}[d_l]<\mathbb{E}[d_{l'}]$ when $l<l'$ (larger processing level requires longer processing time). For the convenience, we denote the set of edges connected to task $v$ by $E_v$ for all task $v$ ($E_v=\{(u,v)|(u,v)\in E\}$), and similarly $E_u$ is set of edges connected to machine $u$.

%We present a formal description of our problem in this section. For a positive integer $i\in\mathbb{N}^+$, we denote $[i]=\{1,...,i\}$. We have a bipartite graph $G=(U,V;E)$, where $U$ is the set of machines and $V$ is the set of repeatable tasks. We are given a set of processing levels $\mathcal{L}=\{1,...,L\}$. For each $u\in U$, we have a discount factor $w_u\in[0,1]$, which describes the discount of utility generated by the depreciation of machine $u$. For each repeatable task $v\in V$, an instance of it can be processed to a level $l\in\mathcal{L}$, which triggers a raw utility $r_{v,l}$. Wlog., we assume for any $v\in V$ and any $l,l'\in \mathcal{L}$ that $l<l'\implies r_{v,l}<r_{v,l'}$. Then we have the net utility gained by processing an instance of $v$ on $u$ to $l$ as $w_u\times r_{v,l}$, which is also the weight of the edge $(u,v)$ if $(u,v)\in E$. This system runs on a finite time horizon $T\in \mathbb{N}^+$. Each processing level $l\in\mathcal{L}$ has a random variable $d_l\in [T]$, which presents the occupation time for processing any task on any machine to level $l$. In other words, if $u$ starts to process $v$ at time $t$, u will become unavailable to any other tasks until time $t+d_l$, where $d_l$ is drawn from a known distribution $D_l$. Wlog., we assume that for any $l,l'\in\mathcal{L}$, $l<l'\implies\mathbb{E}[d_l]<\mathbb{E}[d_{l'}]$.

At each time $t$, task $v$ may arrive with probability $p_{v,t}$. With a probability of $1-\sum_{v\in V}p_{v,t}$, no task arrives at $t$. The set of probability distributions $\{\{p_{v,t}\}_{v\in V}\}_{t\in [T]}$ is known to us in advance (time variant but independent across time).  When a task $v$ arrives, we immediately and irrevocably either assign one machine which is a neighbor to $v$ and is available, or discard $v$. Besides, when we assign task $v$ to machine $u$, we also specify a processing level $l$. When receiving the assignment of task $v$, machine $u$ has two possible actions: with probability $q_e$, $u$ accepts the assignment; with probability $1-q_e$, $u$ rejects the assignment ($e=(u,v)$). Suppose this assignment is specified with processing level $l$, these two actions have two different results. If $u$ accepts this assignment, it immediately gets a reward $r_{u,v,l}$ and becomes unavailable for a random period $d_l$.  A machine $u$ has a limited rejection budget (initialized as $\Delta_u$).
If $u$ rejects this assignment, a rejection-penalty $\theta_l$ is introduced. We assume that $\Delta_u$ and $\theta_l$ are integers. This penalty is taken from the remaining rejection budget of $u$, denoted by $\delta_u$. For convenience, we denote $\theta=\max_{l\in\mathcal{L}}\theta_l$. %Every machine $u$ has an initial budget $\Delta_u$. 
When a machine $u$ runs out of its remaining budget ($\delta_u\leq0$), it is removed from the system immediately and permanently. If a machine $u$ is removed from the system, it receives no more task assignments. %If machine $u$ has a remaining budget of $\delta_u$, we do not allow to assign any task specified with a processing level $l$ larger than $\delta_u$. ($u$ will not a negative remaining budget if the assignment is rejected.)

Each machine has a positive initial budget ($\Delta_u>0$).
Please note we allow $\Delta_u=\infty$ to indicate unlimited rejection. We also allow $\theta_l=1$ to indicate homogeneous rejection penalty (to limit the number of rejections). 
%This is feasible even when machine $u$ is not allowed to make any rejections. In this case, we remove from $u$ all the edges that $u$ may reject ($q_e<1$) and set $\Delta_u$ to 1.

\subsection{Solution Overview}\label{sec:3.1}
Our objective is to maximize the sum reward. We focus on the online setting: we only know the arrival of a task when it arrives. We know the distribution of task arrival in advance and the distribution of occupation time (KAD).

We first construct a linear programming (LP) \texttt{Off} to get an optimal solution $\mathbf{x}^*$ and an upper bound of the offline optimal value, which is referred to as LP(\texttt{Off}). The optimal solution $\mathbf{x}^*$ is then employed to construct our online algorithm. In the meanwhile, the upper bound of the offline optimal value LP(\texttt{Off}) will be set as a benchmark to evaluate the online algorithm, so that we then evaluate the competitive ratio between the performance of online algorithm and the offline optimal value. %The formal definition of competitive ratio is given in the following subsections. 

\subsection{Offline Optimal Value and Competitive Ratio}\label{sec:3.2}

We consider the offline optimization version of the original problem as the benchmark and define the competitive ratio. In the offline setting, the full task sequence $I$ is known in advance. However, we do not know whether a machine will accept or reject an assignment until it happens. We only have the probability of  acceptance $q_e$.
Given a full task sequence $I$, if an offline algorithm maximizes the expected reward, it is an offline optimal algorithm for $I$. This maximized expected reward for $I$ is denoted by OPT($I$). %Among every possible task sequence in $\mathcal{I}$, because each of them arrives with a probability, we then have an expectation of OPT($I$). 
The expected OPT($I$) on every sequence $I$ is $\mathbb{E}_{I\sim\mathcal{I}}[\text{OPT}(I)]$, which is referred to as the \textit{offline optimal value}.


%We have used the offline optimal expected reward $\mathbb{E}_{I\sim\mathcal{I}}[\text{OPT}(I)]$ as a benchmark. 

%{\color{red}Given an online algorithm ALG, the expected overall reward of an online algorithm ALG of a given sequence $I$ is  ALG($I$) . Then we have the expected overall reward of ALG among $\mathcal{I}$ as $\mathbb{E}_{I\sim\mathcal{I}}[\text{ALG}(I)]$. 
{We say that an online algorithm ALG is $\alpha$-competitive if the expected reward obtained by ALG is at least $\alpha$ times the offline optimal value. That is, if $\mathbb{E}_{I\sim\mathcal{I}}[\text{ALG}(I)]\geq\alpha\mathbb{E}_{I\sim\mathcal{I}}[\text{OPT}(I)]$ for any $\mathcal{I}$.}


% we are given the set of probability distributions $\{p_{v,t}\}_{v,t}$. Let $\mathcal{I}$ denote the probability distribution over all possible task sequences. In the offline setting, we assume that the full task sequence $I$ is known in advance. However, the offline algorithm does not know whether a machine will accept or reject an assignment until it happens, but only the probability of this rejection.

% If, given a full task sequence $I$, an offline algorithm maximizes the expected reward, we call it an offline optimal algorithm for $I$. 

% This maximized expected reward for $I$ is denoted by OPT($I$). Among every possible task sequence in $\mathcal{I}$, because each of them arrives with a probability, we then have an expectation of OPT($I$). This expectation of maximized expected reward is denoted by $\mathbb{E}_{I\sim\mathcal{I}}[\text{OPT}(I)]$, and we will also refer to is as the \textit{offline optimal value}. That is, in the offline setting, we only care about the offline optimal value $\mathbb{E}_{I\sim\mathcal{I}}[\text{OPT}(I)]$, not the maximized expected reward OPT($I$) for each specific task sequence $I$, or the specific offline algorithm that achieves it.

\subsection{Linear Programming}\label{sec:3.3}

It is not straightforward to quantify the offline optimal value
$\mathbb{E}_{I\sim\mathcal{I}}[\text{OPT}(I)]$. In what follows, 
we construct an offline LP to get the upper bound of the offline optimal value.  

\begin{align}
    \max_{\substack{x_{e,l,t},\\ \forall e\in E, \\l\in \mathcal{L}, \\t\in[T]}} &\ \displaystyle{\sum_{t\in[T]}\sum_{e\in E}q_e\sum_{l\in\mathcal{L}}}r_{u,v,l} x_{e,l,t}\nonumber\\
    \text{s.t. } & \displaystyle{\sum_{t'<t}\sum_{e\in E_u}q_e\sum_{l\in\mathcal{L}}}x_{e,l,t'}\text{Pr}\{d_l\geq t-t'+1\}  +\displaystyle{\sum_{e\in E_u}q_e\sum_{l\in\mathcal{L}}}x_{e,l,t}\leq1,\ \ (\forall u\in U,t\in [T]),\label{eqn:offst1}\\
    &\displaystyle{\sum_{t\in[T]}\sum_{e\in E_u}\sum_{l\in\mathcal{L}}}x_{e,l,t}\big[\theta q_e\text{Pr}\{d_l>T-t\}+(1-q_e)\theta_l\big]\leq\Delta_u+\theta-1,(\forall u\in U),\label{eqn:offst2}\\
    & 0\leq\displaystyle{\sum_{e\in E_v}\sum_{l\in\mathcal{L}}}x_{e,l,t}\leq p_{v,t},\ \ (\forall v\in V, t\in[T]),\label{eqn:offst4}\\
    & 0\leq\displaystyle{\sum_{l\in\mathcal{L}}}x_{e,l,t}\leq p_{v,t},(\forall v\in V,e\in E_v,t\in[T]),\label{eqn:offst5}\\
    & 0\leq\displaystyle{\sum_{e\in E_u}\sum_{l\in\mathcal{L}}}x_{e,l,t}\leq1,\ \ (\forall u\in U,t\in[T]),\label{eqn:offst6}
\end{align}
This LP is referred to as \texttt{Off}. The optimal solution to \texttt{Off} is $\mathbf{x}^*\defeq \{x_{e,l,t}^*\}$, and the optimal value for the objective function of \texttt{Off} is referred to as LP(\texttt{Off}). LP(\texttt{Off}) is the upper bound for $\mathbb{E}_{I\sim\mathcal{I}}[\text{OPT}(I)]$ (as shown in Lemma below). In addition, $\mathbf{x}^*$ is to be employed in the online algorithm.


%\subsection{LP(\texttt{Off}) is a Valid Upper Bound for the Optimal Offline Value}


In the following Lemma, we show that LP(\texttt{Off}) is a valid upper bound for the offline optimal value $\mathbb{E}_{I\sim\mathcal{I}}[\text{OPT}(I)]$.


%{\color{red} Given a sequence $I$, the optimal offline algorithm  decides the probability that  $v$ is allocated to $u$ with processing level $l$ at $t$. Let $y^I=\{y^I_{e,l,t}\}$ denote the optimal solution given $I$, where $y^I_{e,l,t}$ is a $0-1$ indicates if to allocate $v$ to $u$ ($e=(u,v)$ with level $l$.)} Because $I$ is random, with $I\sim I$, 

\begin{lemma}
\label{lm:1}
 (LP(\texttt{Off}) Upper Bound) LP(\texttt{Off}) $\geq\mathbb{E}_{I\sim \mathcal{I}}[\text{OPT}(I)]$
\end{lemma}


\begin{proof}
Proofs of all Lemmas and Theorems are in the Appendix.
\end{proof}

%In the next subsection, we employ $\mathbf{x}^*$ to construct our online algorithm.

\subsection{Online Machine and Level Assignment (OMLA) Algorithm }\label{sec:3.4}

In this section, we use the optimal solution to \texttt{Off} to construct our OMLA algorithm.

\textbf{Design Overview.} In the online algorithm, we first decide the probability that we choose machine-level pair $(u,l)$ when task $v$ arrives at time $t$. Then we decide whether or not to assign machine $u$ to task $v$ with processing level $l$, by comparing the different expected rewards (of machine $u$) brought by different decisions. We present our online algorithm (OMLA) in Algorithm \ref{alg:online} and we discuss them line by line.

\begin{algorithm}[t!]
\caption{Online Machine and Level Assignment (OMLA) Algorithm}\label{alg:online}
\textbf{Input:} $U$, $V$, $E$, $\{Q^\delta_{e,l,t}\}$, $\{R^\delta_{u,t}\}$, $\mathbf{x}^*$
    \begin{algorithmic}[1]
    
    
    \For{all $t\gets1$ to $T$}
        \If{no task arrives} 
            \State skip
        \Else\ ($v$ arrives)
            \State choose pair $(u,l)$ with probability $x^*_{e,l,t}/p_{v,t}$\label{alg2:choose}
            \If{$u$ is not occupied, $u$ has a positive remaining budget $\delta_u>0$ and $Q^\delta_{e,l,t}\geq R^\delta_{u,t+1}$}\label{alg2:compare}
                \State we assign $(u,l)$ to $v$\label{alg1:9}
                \If{$u$ accepts} 
                    \State draw $d_l$ from $D_l$, $u$ gets occupied for $d_l$\label{alg1:11}
                \Else
                    \State $\delta_u\gets \delta_u-\theta_l$\label{alg1:13}
                \EndIf
            \EndIf
        \EndIf
    \EndFor
        
    \end{algorithmic}
\end{algorithm}

%The online algorithm relies on the optimal solution $\{x^*_{e,l,t}\}_{e,l,t}$ to LP($\texttt{Off}$), and can be divided into two steps. In the first step, we use $x^*_{e,l,t}$ to determine the probability that machine $u$ is chosen with level $l$ when task $v$ arrives at time $t$, where $e=(u,v)$. In the next step, we decide whether or not to assign machine $u$ to task $v$ with level $l$, so that we can have a higher expected reward.\\

\begin{algorithm}[t]
\caption{Calculation of Activation and Baseline Values}\label{alg:QR}
\textbf{Input:} $U$, $V$, $E$, $\mathcal{L}$, $T$, $\{\theta_l\}$, $\{q_e\}$, $\{r_{u,v,l}\}$, $\{D_l\}, \{\Delta_u\}$
\begin{algorithmic}[1]
\State Solve LP(\texttt{Off}) to obtain $\mathbf{x}^*$
\State $\Delta\gets\max\Delta_u$
\For{all $(\delta,u,v,l)$ that $(u,v)\in E, \delta>0$ and $l\in\mathcal{L}$} \label{QR:3}
        \State $Q^\delta_{e,l,T}\gets q_er_{u,v,l}$ \label{QR:4}
\EndFor
\For{all $(\delta,u)$ that $\delta>0$ and $u\in U$}
    \State $a\gets0$ \label{QR:7}
    \For{all $v$ that $(u,v)\in E_u$}
        \State $b\gets0$
        \For{all $l\in\mathcal{L}$}
            \State $b\gets b+x^*_{e,l,T}q_er_{u,v,l}$
        \EndFor
        \State $a\gets a+b$
    \EndFor
    \State $R^\delta_{u,T}\gets a$
\EndFor \label{QR:15}

        \For{$t\gets T-1$ to $1$}
    \For{$(\delta,u)$ that $\delta>0$ and $u\in U$}
        \For{$(v,l)$ that $(u,v)\in E_u$ and $l\in\mathcal{L}$}
            \State $a\gets0$
            
                \If{$\delta\geq\theta_l$} \label{QR:19}
                    \State $b\gets R^{\delta-\theta_l}_{u,t+1}$\label{QR:20}
                \Else\ 
                     $b\gets0$\label{QR:21}
                \EndIf
                \For{$d\gets1$ to $T-t+1$} \label{QR:23}
                    \State $a\gets a+R^\delta_{u,t+d}$Pr$\{d_l=d\}$ \label{QR:24}
                \EndFor\label{QR:25}
                \State $Q^\delta_{e,l,t}\gets q_e(r_{u,v,l}+a)+(1-q_e)b$\label{QR:26}          
    \EndFor
    \State Calculate $R^\delta_{u,t}$ by (\ref{eqn:defR}) \label{QR:R}
\EndFor
\EndFor
    \end{algorithmic}
    \textbf{Output:} $\{Q^\delta_{e,l,t}\}$, $\{R^\delta_{u,t}\}$, $\mathbf{x}^*$
\end{algorithm}

\textbf{OMLA.} Upon the arrival of task $v$, we first choose a machine $u$ and a processing level $l$ with probability $x^*_{e,l,t}/p_{v,t}$ (Line \ref{alg2:choose} in Algorithm \ref{alg:online}). Suppose $u$ has a remaining rejection budget of $\delta$ at $t$. If $u$ has run out of the rejection budget ($\delta\leq0$) or is occupied by a previous task, we do not assign $u$ or assign any other machine to $v$ (Line \ref{alg2:compare} in Algorithm \ref{alg:online}). 
Then, we define the \emph{baseline value} (R-value) of $u$ at $t$ as the expected sum reward of $u$ at and after $t$ without knowing the arrival at $t$, which is denoted by $R_{u,t}^\delta$; we define the \emph{activation value} (Q-value) of $u$ at $t$ as the expected sum reward of $u$ at and after $t$ if $u$ is assigned to $v$ with processing level $l$, which is denoted by $Q_{e,l,t}^\delta$. More details on the derivations of baseline values and activation values will be given shortly. Baseline value and activation value will be compared to make a decision. We compare activation value at $t$ and the baseline value at $t+1$, to decide if an active action at $t$ (making the assignment) is beneficial. 
If the baseline value of $u$ at $t+1$ is larger, we do not assign $u$ and discard $v$; Otherwise, if the activation value is larger at $t$, we assign $u$ to $v$ with $l$ (Line \ref{alg1:9} in Algorithm \ref{alg:online}). When $u$ accepts this assignment, it becomes occupied for a random time $d_l$ (Line \ref{alg1:11} in Algorithm \ref{alg:online}). When $u$ rejects this assignment, a rejection penalty $\theta_l$ is taken from $u$'s rejection budget $\delta$ (Line \ref{alg1:13} in Algorithm \ref{alg:online}).



\textbf{Calculation of  Activation Values and Baseline Values.} Because we focus on the KAD model, we can calculate each activation value and baseline value in advance (before we execute Algorithm~\ref{alg:online}). The calculation is  presented in Algorithm \ref{alg:QR}.  When $u$ has a positive remaining budget ($\delta>0$), the activation value $Q_{e,l,t}^\delta$ consists of two parts: \textcircled{1} With probability $q_e$ ($e=(u,v)$), $u$ accepts the assignment and immediately gets a reward $r_{u,v,l}$ (\ref{eqn:defQ}). After a random occupation time $d_l$, $u$ finishes this task, and its baseline value becomes $R_{u,t+d_l}^\delta$ at $t+d_l$ (Lines \ref{QR:23}--\ref{QR:25} in Algorithm \ref{alg:QR}); \textcircled{2} With probability $1-q_e$, $u$ rejects the assignment and takes a rejection penalty $\theta_l$ on its remaining budget $\delta$, and its baseline value becomes $R^{\delta-\theta_l}_{u,t+1}$ at $t+1$ (Lines \ref{QR:19}--\ref{QR:21}  in Algorithm \ref{alg:QR}). By combining the above two parts, we can calculate the activation value $Q_{e,l,t}^\delta$ as follows
\begin{linenomath}
\begin{align}
Q_{e,l,t}^\delta=&q_e(r_{u,v,l}+\displaystyle{\sum_{d'\in[T-t]}}\text{Pr}\{d_l=d'\}R_{u,t+d'}^\delta)+(1-q_e)R_{u,t+1}^{\delta-\theta_l},\ \ (\delta>0,t\in[T]).\label{eqn:defQ}
\end{align}
\end{linenomath}



Formula (\ref{eqn:defQ}) is calculated in Line \ref{QR:26}  in Algorithm \ref{alg:QR}.
When $u$ has run out of the rejection budget ($\delta\leq0$), it is removed from the market. We set $Q_{e,l,t}^\delta=0$ if $\delta\leq0$ or $t>T$ as boundary values. Because we choose the higher one between the activation value at $t$ and the baseline value at $t+1$, we have the expected reward of the chosen $u$ as $\max\{Q_{e,l,t}^\delta,R_{u,t+1}^\delta\}$. Since the probability that $v$ arrives at $t$ and $(u,l)$ is chosen is $x^*_{e,l,t}$, we can calculate each baseline value $R_{u,t}^\delta$ (Line \ref{QR:R} in Algorithm \ref{alg:QR}) by
\begin{linenomath}
\begin{align}
    R_{u,t}^\delta=&\displaystyle{\sum_{e\in E_u}\sum_{l\in\mathcal{L}}}x^*_{e,l,t}\max\{Q_{e,l,t}^\delta,R_{u,t+1}^{\delta}\}+(1-\displaystyle{\sum_{e\in E_u}\sum_{l\in\mathcal{L}}}x^*_{e,l,t})R_{u,t+1}^{\delta},(\delta>0,t\in[T]).\label{eqn:defR}
\end{align}
\end{linenomath}
We set $R_{u,t}^\delta=0$ if $\delta\leq0$ or $t>T$ as boundary values.


In order to execute our online algorithm, we need to calculate each $Q_{e,l,t}^\delta$ and $R_{u,t}^\delta$ in advance. This can be done with the initial condition at $T$ (Lines \ref{QR:3}--\ref{QR:15} in Algorithm \ref{alg:QR})
\begin{equation}
    \begin{cases}
        Q_{e,l,T}^\delta=q_er_{u,v,l},&\quad\forall e\in E,l\in\mathcal{L},\delta>0,\\
        R_{u,T}^\delta=\displaystyle{\sum_{e\in E_u}\sum_{l\in\mathcal{L}}}x^*_{e,l,T}q_er_{u,v,l},&\quad\forall u\in U,\delta>0.
    \end{cases}\label{eqn:11}
\end{equation}
We present the algorithm to calculate each $Q_{e,l,t}^\delta$ and $R_{u,t}^\delta$ in Algorithm \ref{alg:QR}. %We note that the expected overall reward of the online algorithm is equal to $\sum_{u\in U}R^{\Delta_u}_{u,1}$.

%\subsection{Complexity Analysis of Algorithms}\label{sec:3.5}

%See Appendix for the complexity analysis.




==> [arXiv] OMLA (For Publish)/Sections/RelatedWork.tex <==
\section{Related Work}\label{sec:2}

One category of works related to this paper is \textit{Online Bipartite Matching}, where the system needs to assign offline machines to online tasks to maximize the utility~\cite{RN66}. One subcategory of works focuses on the adversary arrival order~\cite{RN64}, and another subcategory assumes known adversarial distribution (KAD)~\cite{RN47,RN65} or known identical independent distributions (KIID)~\cite{RN68}, where task arrival  follows known distributions. Motivated by real-world scenarios, \cite{RN84} and \cite{RN49} studied the case that machines are reusable, and \cite{RN52,RN53,RN62} studied the case that machines can reject task assignment. \cite{RN51} studied both reusable machines and rejections. Other topics studied in this field include fairness for task assignment~\cite{RN50,RN54}, multi-unit demand (a task may need multiple machines to process)~\cite{RN46,RN55}, and multi-capacity agent (a machine can process multiple tasks)~\cite{RN80,RN56}. However, there is no existing work considering controllable processing time in the online bipartite matching
problem. A majority part of \cite{RN51} can be regarded as a special case of our work when controllable processing time is not considered.  It gives a $1/2$-competitive algorithm when each offline machine can reject unlimited times, and a $\Delta/(3\Delta-1)$-competitive algorithm when each machine can reject no more than $\Delta$ times. Interestingly, our proposed algorithm also gives the same competitive ratios, but with substantially more complicated designs and analyses. To this end, a key conclusion derived in our paper is that the competitive ratio is ``insensitive'' to the processing levels.  Please note that another work~\cite{RN79} studied controllable reward and different arrival probabilities, where the assignment impacts reward and arrival probabilities, which is different from controllable processing time
in nature. Online bipartite matching is leveraged to solve many real-world problems other than machine allocation, such as ride-sharing~\cite{RN47,RN49,RN50}, crowd-sourcing~\cite{RN46,RN99,RN79} and AdWords~\cite{RN78}. Still none of the existing work considered controllable processing time. 


% where the worst case performance is studied when the arrival order is adversary. Online bipartite matching with known adversarial distribution (KAD)  was studied in [43].%, and the  the prophet-inequality i [44][45] as a special case. 
% In addition to the arrival assumptions of KAD and adversarial order, there are other important arrival assumptions for online matching problems. Under known identical independent distributions, the arrival distribution of agents is time-invariant (eg., online-matching [48]). Under unknown distributions, at each time, the arriving task is sampled from an identical but unknown distribution (eg., resource-allocation [49]). Please refer to [47] for a detailed survey. 

% [46] was the first to consider the online bipartite matching problem where an offline machine may reject an assignment with a probability, and each machine is allowed to reject unlimited times (machine rejection). [6] was the first to consider the online bipartite matching problem where offline machines return to the system after a limited occupation time (machine reusability), and gives a $1/2$-competitive algorithm for known adversarial distribution. [8] considers the online bipartite matching problem with both machine reusability and machine rejection. [8] gives a $1/2$-competitive algorithm when each offline machine can reject unlimited times, and a $\Delta/(3\Delta-1)$-competitive algorithm when each machine can reject no more than $\Delta$ times. However, none of these work considered controllable processing level. [5] considers the controllable reward in the online bipartite matching. However, [5] is different from ours, because they control the reward by controlling the online task that a machine is assigned to, while we control the reward by controlling the processing level specified with the assignment.
%Examples include:  under the condition of known adversarial distributions [3][4][6][8];  under the condition of known independent identical distributions [7][8][9][10][27];  offline agents may reject assignments [7][8][9][10];   offline agents are reusable [1][2][4][6][8]; the objective is fairness [7][11][12]; tasks are with multi-unit demand (a task should be processed by multi-machines simultaneously) [1][8]; agents are with multi-unit capacity and tasks arrive in batches [3][13][14]. However, none of the work considered controllable processing time.One similar model to ours is [8], where both reusable offline agents and stochastic rejection are considered. [8] designs an online algorithm with a $1/2$-competitive ratio for unlimited rejection cases and a $\Delta/(3\Delta-1)$-competitive ratio when each offline agent has an initial rejection budget no more than $\Delta$. However, [8] does not consider the controllable processing times in the problem. 


%One application area is ride-sharing, where the online tasks are passenger requests and offline machines are taxis [51]. Plenty of works have discussed the ride-sharing under online bipartite matching problem (eg., [3][6][7]). Another application area is crowd-sourcing, where online tasks are jobs and offline machines are workers [36]. The online bipartite matching problem in crowd-sourcing is also well-studied (eg., [1][4]). However, none of existing work mentions the controllable processing levels in the above applications. In the ride-sharing scenario, the driver can choose to go through toll roads to reduce the processing time and the reward. In the crowd-sourcing scenario, a worker can choose to finish the job quicker with a lower quality and reward. To our best knowledge, we are the first to address the controllable processing levels in these two application areas.

%Another relevant work considers the cases that the reward and the arrival probability of online tasks may vary with the density of offline agents in an area [5]. However, [5] considers the controllable reward and the controllable arrival probabilities, which is different the controllable processing levels. To the best of our knowledge, there is no existing work considering controllable processing levels in the online bipartite matching problem.   

%Among the studies of bipartite matching problems, there are several applications areas considered: ride-sharing [3][5][6][7], crowd-sourcing [1][4][5][6] and (resource) scheduling problem [37][38]. All the above studies focuses on allocating limited resources (eg., taxis [3][5][6][7]) to arriving demands (eg., passengers [3][5][6][7]) in an online manner. However, all the above studies do not consider the controllable processing levels, which is addressed in our work. 


Another category of works related to this paper is \textit{Controllable Processing Time}. Controllable processing time is studied in the context of scheduling. We can reduce the processing time of a job at a cost of reduced processing reward~\cite{RN68,RN69}. \cite{RN70}, \cite{RN71} and \cite{RN72} study single machine scheduling. \cite{RN75} and \cite{RN77} study multiple parallel machine scheduling. \cite{RN76} employs bipartite matching to analyze multiple parallel machine scheduling. The above works focus on the offline scheduling problem. %In the offline machine scheduling problem, the processing time of each processing level is deterministic, and this is different from our stochastic occupation times. 
\cite{RN73} and \cite{RN74} study online scheduling with controllable processing time. \cite{RN73} focuses on single machine scheduling and \cite{RN74} focuses on the flow shop scheduling.
Controllable processing time is also analyzed in the context of stochastic lot-sizing problem. We can compress the production time with extra cost, so that a better performance of planning can be obtained~\cite{RN57,RN82,RN59}. These works optimize the performance in an offline manner. To the best of our knowledge, no existing work considered controllable processing time for the bipartite matching problem. 

%The controllable processing levels studied in the above two areas is similar to ours, where the processing time can be reduce at a cost of reduced reward. However, the controllable processing levels in the bipartite matching problem is different, because: 1) in stochastic lot sizing problem, there is no bipartite graph; 2) in machine scheduling problem, competitive ratio is not used as a performance measure. 

%Another related field is \textit{Controllable Processing Levels}. Controllable processing levels has gained much attention in two areas: stochastic lot-sizing Problems and machine scheduling Problems. In stochastic lot-sizing problem, the controllable processing levels allow to reduce the processing time of the product in return for extra cost [15][18][25]. In machine scheduling problems, the controllable processing levels allow allows a task to be processed with different levels, so as to gain different rewards and to spend different time [16][17][19][20]. Controllable processing levels is studied with different focuses in machine scheduling problems: single machine scheduling [16][20][24]; multi-machine scheduling [17][21][22][23]; optimization of total tardiness (instead of total reward) [21][23][24]; the application in Deep Neural Network Early Exit [16][20]. However, all those above works are different from ours, because none of them considers the controllable processing levels in the bipartite matching problem.

%Ride-sharing is an important application area of this work, which is also an active research area of other fields. Some works discuss the pricing strategy in ride-sharing towards a game-theory approach [27][29][30][31]. Some other works focus on privacy protection in ride-sharing scenarios [32][33][34][35]. Our problem focuses on the online task assignment in ride-sharing, which also is addressed by many other work of online bipartite matching problem [3][5][6][7][8][11][13][14]. However, none of these works consider the ride-sharing problem where toll influences the transportation time and rewards as we do.




